3D Correlations in the Lyman-$\alpha$ Forest from Early DESI Data

We present the first measurements of Lyman-$\alpha$ (Ly$\alpha$) forest correlations using early data from the Dark Energy Spectroscopic Instrument (DESI). We measure the auto-correlation of Ly$\alpha$ absorption using 88,509 quasars at $z>2$, and its cross-correlation with quasars using a further 147,899 tracer quasars at $z\gtrsim1.77$. Then, we fit these correlations using a 13-parameter model based on linear perturbation theory and find that it provides a good description of the data across a broad range of scales. We detect the BAO peak with a signal-to-noise ratio of $3.8\sigma$, and show that our measurements of the auto- and cross-correlations are fully-consistent with previous measurements by the Extended Baryon Oscillation Spectroscopic Survey (eBOSS). Even though we only use here a small fraction of the final DESI dataset, our uncertainties are only a factor of 1.7 larger than those from the final eBOSS measurement. We validate the existing analysis methods of Ly$\alpha$ correlations in preparation for making a robust measurement of the BAO scale with the first year of DESI data.

==> alternative_dla.tex <==
\section{Alternative DLA catalogue} \label{app:alt_dla}

In section \ref{sec:pixmask} we discuss DLAs, why we mask them and how they are identified. Here we outline the differences between the two DLA catalogues that were considered for our baseline analysis. In the "baseline" and "alternative" cases 7\% and 20\% of our \lya forests have DLAs respectively. The difference in number is due to the selection on the confidence of the convolutional neural network DLA finder, where in the alternative analysis we require a lower confidence for a DLA detection. In figure \ref{fig:dla_corr_comp} we show the  

\begin{figure}
\hspace*{-0cm} 
   \centering  
   \includegraphics[scale=0.4]{figures/dla_corr_conpare.png}
   \vspace*{-10mm}
   \caption{The ratio of errorbars on the \lya auto-correlation produced using two different DLA catalogues.}
   \label{fig:dla_corr_comp}
\end{figure}



\begin{figure}
\hspace*{-2cm} 
   \centering  
   \includegraphics[scale=0.3]{figures/dla_corn_plots.png}
   \caption{A comparison of selected parameters in our baseline fit on the combined auto+cross correlations, using two different DLA catalogues in the flux transmission field measurement. DLA baseline is the catalogue used to produce the results in our baseline fit (table \ref{table:bestfit}) where 7\% of \lya forests have at least one DLA. DLA alternative has a lower confidence requirement for detected DLAs, and thus 20\% of \lya of forests in that catalogue have a DLA. The selected parameters are those for which changing to the alternative DLA catalogue had the most effect.}
   \label{fig:dla_corn_plots}
\end{figure}



==> blinding.tex <==
%\section{Appendices}\label{sec:appendices}

%\section*{Appendix A: Blinding}\label{sec:AppA}
%The fact that there are around $2 \times$ fewer pixels in the Ly$\beta$ forest combined with the increased noise and absorption fluctuations (from e.g. Ly$\beta$ absorption) means that in general the variance of this measurement is around 3 $\times$. In figure \ref{fig:nb_nb_nb_auto} we show the number of pairs in the $Ly\alpha$($Ly\alpha$) auto correlation as a function of ($r_\parallel,r_\perp$) and the ratio of the number of pairs in DESI EDR to eBOSS DR16. We have divided the left plot by transverse separation for visualisation purposes, since our pixel number increases strongly with $r_\perp$. and there is little change with $r_\parallel$. From the pixel count plot we can see that we have a drop in pixels in the lowest (0-4$h^{-1}Mpc$) transverse bin. This is because of collisions between neighbouring fibres on the DESI focal plane*?. As mentioned previously, we also ignore correlations from pixel pairs within the same forest. We also note a "dip" in the pixel count in the second lowest line-of-sight bin ([4,8]$h^{-1}Mpc$). *why?* On the right side of figure \ref{fig:nb_nb_nb_auto} we see the ratio of pixel pairs from DESI to DR16, and note the much higher ratios at low separation. This is because of the large high redshift quasar target density in DESI compared to eBOSS ($\sim 60 deg^2$ compared to $\sim 25 deg^2$ for $z>2$). It is also reassuring that with a small early data set from DESI we can already perform worthwhile analysis of Ly$\alpha$ correlations because of the relatively high pixel pair ratio, especially at smaller scales.

%In figure \ref{fig:nb_nb_nb_cross} we again show the number of DESI EDR $QSO-Ly\alpha$ pairs divided by $r_\perp$ as a function of ($r_\parallel,r_\perp$) and the ratio of pairs in DESI EDR to eBOSS DR16 across the same range. From the first plot (left) we can see a strong asymmetry between the number of pairs at -ve and +ve separations because the Ly$\alpha$ have a higher mean redshift. Interestingly we see this same trend in the righthand plot, which implies an even stronger pair asymmetry in our data than in eBOSS DR16.

%\begin{figure}
%\hspace*{-2cm} 
   % \centering  
    %\includegraphics[scale=0.5]{figures/nb_nb_nb_auto.png}
    %\caption{pixels pixels pixels}
  %  \label{fig:nb_nb_nb_auto}
%\end{figure}


%\begin{figure}
%\hspace*{-2cm} 
 %   \centering  
 %   \includegraphics[scale=0.5]{figures/nb_nb_nb_cross.png}
%    \caption{pixels pixels pixels}
%    \label{fig:nb_nb_nb_cross}
%\end{figure}

\subsection{B: Minimum Fit Separation}

We make the choice to set the lower limit on our Ly$\alpha$ x quasar fit to r$_{min}$=30h$^-1$Mpc, based on results from the AbacusSummit mocks [Boryana].... explain***

\begin{figure}
\hspace*{-0.5cm} 
    \centering  
    \includegraphics[scale=0.5]{figures/cross_wedge_fit_rmin.png}
    \caption{preliminary}
    \label{fig:cross_wedge_fit}
\end{figure}

\begin{figure}
\hspace*{-0.5cm} 
    \centering  
    \includegraphics[scale=0.5]{figures/1d_cross_fit_rmin.png}
    \caption{preliminary}
    \label{fig:cross_1d_fit}
\end{figure}

\begin{figure}
\hspace*{-0.5cm} 
    \centering  
    \includegraphics[scale=0.5]{figures/rmintest_sigma_v.png}
    \caption{preliminary}
    \label{fig:sigma_v}
\end{figure}


==> results.tex <==
\section{Measuring the Auto and Cross Correlation} \label{sec:results}



\subsection{Measurement of the Lyman-$\alpha$ auto-correlation}

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/cf_wedges_all.png}
    \caption{Measured \lya\ auto-correlation in the usual 4 wedges.}
    \label{fig:cf_wedges_all}
\end{figure}

In Figure \ref{fig:cf_wedges_all} we whow the measured wedges.
\AFR{Should add LYB region, maybe compare to eBOSS}


\subsection{Measurement of the QSO x Lyman-$\alpha$ cross-correlation}

Show the measured wedges in the LYA and LYB region, maybe compared to eBOSS?

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/xcf_wedges_all.png}
    \caption{Measured QSO x \lya\ cross-correlation in the usual 4 wedges.}
    \label{fig:xcf_wedges_all}
\end{figure}

In Figure \ref{fig:xcf_wedges_all} we whow the measured cross-correlation.
\AFR{Should add LYB region, maybe compare to eBOSS}

\subsection{Using smaller separations}



